The Case for a Legal Compliance API for the Enforcement of the EU's Digital Services Act on Social Media Platforms

In the course of under a year, the European Commission has launched some of the most important regulatory proposals to date on platform governance. The Commission's goals behind cross-sectoral regulation of this sort include the protection of markets and democracies alike. While all these acts propose sophisticated rules for setting up new enforcement institutions and procedures, one aspect remains highly unclear: how digital enforcement will actually take place in practice. Focusing on the Digital Services Act (DSA), this discussion paper critically addresses issues around social media data access for the purpose of digital enforcement and proposes the use of a legal compliance application programming interface (API) as a means to facilitate compliance with the DSA and complementary European and national regulation. To contextualize this discussion, the paper pursues two scenarios that exemplify the harms arising out of content monetization affecting a particularly vulnerable category of social media users: children. The two scenarios are used to further reflect upon essential issues surrounding data access and legal compliance with the DSA and further applicable legal standards in the field of labour and consumer law.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> sections/data-needed.tex <==
\section{Data needed for digital enforcement in the two scenarios}


\subsection{General barriers to digital enforcement}



\textbf{Data needed}: What could authorities need in order to audit/enforce local child labour laws according to the provisions cited above?  
Ideally, imagine a system in which platforms report to legal authorities (periodically or upon request) information that would allow authorities to flag behaviour inconsistent with child labour laws. 
We need to: 
\begin{enumerate}
    \item Identify when a child is involved in creating the content (via self-disclosure). This information is not currently disclosed when an account is created (\ainote{to check!!!! Can we give some specifics?}).   
    We need to distinguish between who opened the account and who ``works'' for the account. \ainote{note that it is irrelevant how popular the account is, as the focus here is child labour.} 
    At a minimum, platforms should be required (?) to provide to legal authorities a list of child influencer accounts on the platform (per territory (country)?)
    
    \item Since contracts are private, we need a different way of identifying monetised efforts. This can be done by proxy -- make available hashtags promoted by brands. The challenge is that platforms do not have direct information about the hashtags promoted, instead they could use their in-house analytics to infer trending hashtags and thus promotion campaigns. Trending hashtags can reveal more than marketing campaigns, such as political or disinformation campaigns. 
   \ainote{to rewrite the following:} A way for auditors to review the contracts between brands and child (where available). Note that platforms are not supposed to be part of the contract or to have access to it, but they could be required to report the permit number of the child content creator. This permit number can be used to connect the user account on the platform with a contract that resides in the archives of whatever entity/part of bureaucracy. Information about the mandatory obligations included in private contracts concluded between brands and child influencers would also be useful.\ainote{does this belong to labour law/contract templates or to platforms' requirements for providing data?} --- 
    
    \item Information from platforms related to actual content created (as a way to estimate intensity of labour), such as duration of the content posted and frequency of new posts. This can be used to check consistency between labour contract and apparent effort invested by child creator. Note that a child creator could be part of multiple contracts for multiple brands on multiple platforms. \ainote{note this point raises the issue of the need for a platform agnostic API, such that information from multiple platforms is easily collected and aggregated)}
    
    \item add parameters to make reporting more transparent re Art 4(3) from the law
    
\end{enumerate}

Based on this information, "authorities" can process the data and identify particular accounts that they might want to investigate more closely. The status quo is ... \ainote{Catalina?}.

%\tbnote{This question raises many points we need to clarify (maybe on a different section?)}

%\tbnote{What do authorities need -> We can approach this as ``what authorities need to automatise whatever they currently do'' or as ``how can authorities do this more efficiently assuming they had access to the data we are talking about?''. In any case, we should discuss what these authorities do in practice (e.g. describe the manual process of going through some videos), or at least what they ``look'' at -- i.e., what would be the relevant features for them?}



(How will this transparency distort user and platform behaviour?)


Note that even if this data can be collected via API or from intermediary companies, they are not guaranteed to be accurate because the platform has the "truth". 


\subsection{Scenario 2}

\textbf{Scenario 2}: 

\ainote{what's needed: to connect content to inferred age of audience (not declared); -- should that connection be disclosed for auditing?}

Data that could be of interest:
\begin{itemize}
    \item what is the (declared) under-age following (per country) per content? Do we also want the under-age following per ads? 
    
    \item What is the \emph{inferred} under-age following per country per content? -- note that this needs processing of platform data, perhaps classification algorithm to infer when a grown up account is used by a child. This can be done by using the inferred/declared age of the content creator, under the assumption that teens will target a teens audience, etc. Note that requiring platforms to track the link between inferred age and content viewed might make the platforms more responsible?
    
    \item disclosure of content typology according to the legal classifications of harmful content in the local legal context.  (e.g., fast-food, unhealthy behaviour (guns, anorexia, ...). This would be a difficult (impossible?) task, prone to algorithmic and cultural biases in classifying harmful content. Note that some content can be clearly defined as harmful, while there are many types of content that are debatable in terms of harm. -- specify community guidelines \ainote{how do we make this actionable? what would be the progress/contribution here?} 
\end{itemize}



\textbf{Data needed}:

Exposure/manipulation of kids to ads. 2 objectives: 1) identify ads; 2) identify when target audience is under age

\begin{itemize}
    \item image/object recognition + text mining for undisclosed brands advertising
    \item frequency of posting of undisclosed brands
    \item target audience: kids or not
\end{itemize}






What could authorities need in order to audit/enforce local child labour laws according to the provisions cited above?  
Ideally, imagine a system in which platforms report to legal authorities (periodically or upon request) information that would allow authorities to flag behaviour inconsistent with child labour laws. 

    \item differentiating between commercial and non-commercial users to allocate legal obligations; 
    
   \ainote{to rewrite the following:} A way for auditors to review the contracts between brands and child (where available). Note that platforms are not supposed to be part of the contract or to have access to it, but they could be required to report the permit number of the child content creator. This permit number can be used to connect the user account on the platform with a contract that resides in the archives of whatever entity/part of bureaucracy. Information about the mandatory obligations included in private contracts concluded between brands and child influencers would also be useful.\ainote{does this belong to labour law/contract templates or to platforms' requirements for providing data?} ---     
    
    
    \item identifying connections at scale between various categories of users to map and visualise the ecosystem in which they operate. 
    
  
  
disclosure of content typology according to the legal classifications of harmful content in the local legal context.  (e.g., fast-food, unhealthy behaviour (guns, anorexia, ...). This would be a difficult (impossible?) task, prone to algorithmic and cultural biases in classifying harmful content. Note that some content can be clearly defined as harmful, while there are many types of content that are debatable in terms of harm. -- specify community guidelines
\ainote{how do we make this actionable? what would be the progress/contribution here?} 
    


 
    We need to distinguish between who opened the account and who ``works'' for the account. \ainote{note that it is irrelevant how popular the account is, as the focus here is child labour.} 
    At a minimum, platforms should be required (?) to provide to legal authorities a list of child influencer accounts on the platform (per territory (country)?)
    
Since contracts are private, we need a different way of identifying monetised efforts. This can be done by proxy -- make available hashtags promoted by brands. The challenge is that platforms do not have direct information about the hashtags promoted, instead they could use their in-house analytics to infer trending hashtags and thus promotion campaigns. Trending hashtags can reveal more than marketing campaigns, such as political or disinformation campaigns. 

    
Information from platforms related to actual content created (as a way to estimate intensity of labour), such as duration of the content posted and frequency of new posts. This can be used to check consistency between labour contract and apparent effort invested by child creator. Note that a child creator could be part of multiple contracts for multiple brands on multiple platforms. \ainote{note this point raises the issue of the need for a platform agnostic API, such that information from multiple platforms is easily collected and aggregated)}
    
add parameters to make reporting more transparent re Art 4(3) from the law


Based on this information, "authorities" can process the data and identify particular accounts that they might want to investigate more closely. The status quo is ... \ainote{Catalina?}.


==> sections/discussions.tex <==
\section{Discussions}




%To mention that things are more nuanced when we consider: 

%* territoriality -- laws in different countries are different, what are the platforms to do?

%* capabilities theory -- Martha Nussbaum 

%What we can get right vs what we need: discuss lack of transparency of platforms etc:

%\tbnote{What authorities can get from platforms -> I see this as two separate discussions, maybe on different sections: First, what we can get from platforms right now (which would include criticism about the lack of transparency, issues with sharing etc.). Second, what we need (or should be able) to get for legal compliance. Then we need to define ``'data'' more clearly. Are we talking about raw data (e.g. the videos themselves) or processed data (e.g. a flag indicating whether the video has a child on it). If it's processed data, we need to discuss who should be responsible for running the models/methods that do this processing (what Anda talked about last time we met).}

%Discussion points: what are the costs that the platforms need to invest to comply with legislation? What are the requirements that platforms enforce when opening user accounts to correctly record user age/location? (e.g., upload ID -- trouble as in voting in US). 

%Possible harms and potential misuses of these data. 

%Distinction between legal standard and harm (e.g. influencer disclosures?)

%Can these data be "gamed"/faked by the creators? What are the exceptions (e.g. old content repost)? 
    %(How will this transparency distort user and platform behaviour?)

%Need for a platform-agnostic standard -- authorities should not need to go to each platform individually to get the required data.

==> sections/todo.tex <==
\section{To Do}


- define enforcement and investigation


 





\ainote{to define API; what are the practical benefits of an API; sm companies already have such apis}

\ainote{why we need a legal API}

\ainote{to add references wherever approriate}




\ainote{Anda will put these refs in other places as needed}
 talks about how not to trust platform's API.
\cite{DBLP:conf/icwsm/Tufekci14}









()








\begin{enumerate}
    \item Catalina is writing scenarios with the harms done: harms; legal issues; data needed.  
    \item harmonize child; harmonize legal enforcement
    \item 
\end{enumerate}



\subsection{Scenario 2: Harmful content for the health of minors}

Children on social media can be creators, but also audiences which have been traditionally offered special protections under media laws, due to their particular vulnerability in media exposure.  The past decade has seen a rise in interest for the prohibition, both at national and European level, of the advertising of unhealthy foods. Consumer studies in various European countries such as Spain or France show that up to 89\% of food products advertised to children have least favourable nutrition scores (and are thus considered generally unhealthy). In comparison, the rate of products of similar low nutrition value advertised to adults was up to 43\%. 

Social media content monetization amplifies the risks of exposing children to unhealthy food advertising in two ways. First, advertising is much more diverse on social media, and it includes platform ads (such as ads displayed through AdSense), but also influencer marketing (e.g. native advertising in social media content). For the first category, platforms are the sole responsible entities for filtering the content and providers of ads. Some platforms openly share their ad libraries. For instance, TikTok's Top Ads Library is supposed to help advertisers investigate the performance of selected ads, in order to get inspiration for their own campaigns. %https://ads.tiktok.com/business/creativecenter/inspiration/topads/pc/en. 
Another example is Meta's Ad Library, created as a transparency tool after waves of backlash against political ads and potentially discriminatory ads facilitated by the Meta advertising ecosystem. 
%https://www.facebook.com/ads/library/?active_status=all&ad_type=political_and_issue_ads&country=NL&media_type=all. 
Regarding the second category, content creators may engage with brands in the course of endorsement or barter transactions. A clear practical example is offered by energy drink companies which have been sponsoring live streams on Twitch or content on Instagram by influencers who are popular with minors. 

%https://www.beuc.eu/publications/beuc-x-2021-084_food_marketing_to_children_needs_rules_with_teeth.pdf

The most recent regulatory reform at European level, the updated Audiovisual Media Services Directive (AVMSD), stipulates in its Art. 6a that 'audiovisual media services provided by media service providers [...] which may impair the physical, mental or moral development of minors are only made available in such a way as to ensure that minors will not normally hear or see them'. The Preamble gives more specific indications of the health concerns around advertising targeting children and minors. Recital 28 supports co-regulatory instruments such as codes of conduct, in order to 'effectively reduce the exposure of children to audiovisual commercial communications regarding foods and beverages that are high in salt, sugars, fat, saturated fats or trans-fatty acids or that otherwise do not fit those national or international nutritional guidelines.' More specifically, Recital 29 refers to the reduction of 'the exposure of children and minors to audiovisual commercial communications for alcoholic beverages.' 

As the AVMSD left generous discretion for the implementation by Member States, for a more concrete understanding of the applicable rules to food advertising for children and minors it is necessary to further investigate relevant national legal frameworks. In the Netherlands, a new code of conduct was introduced in 2019 on the topic of advertising food items (Reclamecode Voor Voedingsmiddelen 2019 - RVV). The RVV also includes specific provisions on advertising directed at children. Art. 8.1 RVV establishes a general prohibition on the advertising of food items to children up to and including 12 years, with three exceptions: a) advertising for food items undertaken in cooperation with or supported by the government and/or another recognized authority in the field of nutrition, health and/or physical exercise; b) packaging and point-of-sale material; and c) advertising directed at children from 7 up to and including 12 years of age, for foods which meet the nutritional criteria established by the RVV. Out of these three exceptions, only a) and c) are relevant for advertising which can be done on social media, and would thus need monitoring for legal compliance. 

In addition, the RVV also sets out the context in which this advertising may take place. Art. 8.4 states that advertising food products is considered to target children when: a) it appears in media which is specifically aimed at children up to 12 years according to generally accepted market research; or b) it appears in media not specifically aimed at children up to 12 years, but according to generally accepted market research this demographic constitutes at least \%25 of the audience. The RVV also acknowledges the difficulty of applying these standards to social media. However, Art. 8.4 is accompanied by a note that indicates a set of criteria which can be used to determine user profiles on social media for the purpose of establishing if advertising appears as or on content that is considered to target children. The list of non-exhaustive criteria includes:
\begin{itemize}
    \item Language use: is a tone or choice of words used that is specifically aimed at children?
    \item Design and animation: are design, animation, cartoons, fantasy images or coloring pages used specifically for children?
    \item Games and playful activities: are games, toys, crafting tips offered specifically geared toward children?
    \item Children's idols: are children's idols, such as licensed media characters, popular with children used and, if so, what age target group are those children's idols aimed at?
\end{itemize}

%https://www.reclamecode.nl/nrc/rvv2019/
%https://www.reclamecode.nl/wp-content/uploads/2019/02/Voedingskundige-criteria-Reclame-gericht-op-kinderen-7-tot-en-met-12-jaar-d.d.februari-2019.pdf
%https://www.foodwatch.org/nl/current-nieuws/2020/mag-niet-gebeurt-wel-paw-patrol-frozen-en-minions-in-het-supermarktschap/?cookieLevel=not-set
